ASP:A Fast Adversarial Attack Example Generation Framework based on Adversarial Saliency Prediction

With the excellent accuracy and feasibility, the Neural Networks have been widely applied into the novel intelligent applications and systems. However, with the appearance of the Adversarial Attack, the NN based system performance becomes extremely vulnerable:the image classification results can be arbitrarily misled by the adversarial examples, which are crafted images with human unperceivable pixel-level perturbation. As this raised a significant system security issue, we implemented a series of investigations on the adversarial attack in this work: We first identify an image's pixel vulnerability to the adversarial attack based on the adversarial saliency analysis. By comparing the analyzed saliency map and the adversarial perturbation distribution, we proposed a new evaluation scheme to comprehensively assess the adversarial attack precision and efficiency. Then, with a novel adversarial saliency prediction method, a fast adversarial example generation framework, namely "ASP", is proposed with significant attack efficiency improvement and dramatic computation cost reduction. Compared to the previous methods, experiments show that ASP has at most 12 times speed-up for adversarial example generation, 2 times lower perturbation rate, and high attack success rate of 87% on both MNIST and Cifar10. ASP can be also well utilized to support the data-hungry NN adversarial training. By reducing the attack success rate as much as 90%, ASP can quickly and effectively enhance the defense capability of NN based system to the adversarial attacks.

==> category.tex <==
\vspace{-6mm}
\category{\vspace{-1mm}C.1.3}{Special-Purpose and Application-Based Systems}{Real- Time and Embedded Systems}
\vspace{-4mm}
\terms{\vspace{-1.5mm}Design, Management, Performance}
\vspace{-4mm}
\keywords{\vspace{-1.5mm}OLED, Camera, Video streaming, Mobile device}
\vspace{-2mm}

